Efficient Multi-word Compare and Swap

Atomic lock-free multi-word compare-and-swap (MCAS) is a powerful tool for designing concurrent algorithms. Yet, its widespread usage has been limited because lock-free implementations of MCAS make heavy use of expensive compare-and-swap (CAS) instructions. Existing MCAS implementations indeed use at least 2k+1 CASes per k-CAS. This leads to the natural desire to minimize the number of CASes required to implement MCAS. We first prove in this paper that it is impossible to "pack" the information required to perform a k-word CAS (k-CAS) in less than k locations to be CASed. Then we present the first algorithm that requires k+1 CASes per call to k-CAS in the common uncontended case. We implement our algorithm and show that it outperforms a state-of-the-art baseline in a variety of benchmarks in most considered workloads. We also present a durably linearizable (persistent memory friendly) version of our MCAS algorithm using only 2 persistence fences per call, while still only requiring k+1 CASes per k-CAS.

==> tex/optimality.tex <==
\section{Reaching Optimality}\label{sec:optimality}

%The attentive reader will notice that our algorithm, presented in Section~\ref{sec:algos}, uses $k+1$ \cas{} instructions to implement a $k$-word \mcas{}; the persistent version of our algorithm additionally uses $2$ persistence fences for the same task. 
In this section, we describe how our algorithm can be modified to become optimal, both in terms of \cas{} instructions and in terms of persistence fences~\cite{cohen18}.
Intuitively, the crucial change consists in removing the status field of \mcasdescriptor{} (and thus of the \cas{} to set the status), while ensuring the status of an operation is never ambiguous.

We introduce two new notions, compared to our algorithm in Section~\ref{sec:algos}.
First, we introduce \textit{failure descriptors}, which are structures with the following fields: a pointer $P$ to another descriptor $D$, an address $W$ and a value $V$.
As explained below, a failure descriptor is created and used to mark the failure of the \mcas{} operation corresponding to $D$.
We distinguish between a failed and a non-failed (regular) descriptor by stealing one of the least-significant bits in a pointer.
(Alternatively, we can add an immutable \texttt{type} field in the descriptor structures initialized during the construction of a descriptor).
Second, when applying an \mcas{} $M'$ after a previous \mcas{} $M$, we do not remove pointers to $M$, but rather change the old/new value (depending on whether $M$ succeeded or failed) in $M$'s descriptor to point to $M'$. 
This effectively creates a \textit{chain} of descriptors for each memory word.
 
The new algorithm works as follows.  
Just like before, an \mcas{} $M$ attempts to lock (install pointers to an \mcasdescriptor{} in) the target words one-by-one, using one \cas{} instruction per locked word.
$M$ is successful if it manages to lock all its words.
If $M$ finds a value $V$ different from the expected value $E$ in one of the target words $W$, $M$ creates a failure descriptor (with a pointer $D$, address $W$ and value $V$), and installs (with \cas{}) a pointer to this failure descriptor into $W$. 
This has the effect of failing $M$.
Thus, a successful \mcas{} operation uses exactly $k$ CAS instructions, while a failed \mcas{} uses at most $k$ CAS instructions. 

Like before, when a (read or another \mcas{}) operation $M'$ finds an \mcas{} $M$ in progress, $M'$ attempts to determine $M$'s status by reading though all its words (which are sorted by their target addresses, as before).
Note that $M'$ might need to traverse chains of descriptors for that and help them recursively.
If $M'$ finds all of $M$'s target words to be locked, then $M$ is successful, and $M'$ proceeds to use the corresponding new values.
If $M'$ finds a pointer to a failure descriptor $F$ that belongs to $M$ (i.e., $F$ has a pointer to $M$), $M$ is failed and $M'$ proceeds to use the corresponding old value (which is the value $F.V$ for the word that has a pointer to $F$ or the expected value for a word that has a pointer to $M$).
Otherwise (if $M$ is still active), $M'$ helps to complete $M$, either by locking the remaining words, or \cas{}-ing a pointer to a failed descriptor.

As described above, this new algorithm does not use a status field, thus eliminating the need for a persistence fence to ensure the status is persistent. As such, only one fence is required, to ensure the persistence of all locked words (in the case of a successful \mcas{}), or the persistence of a pointer to the failure descriptor (in the case of a failed \mcas{}). As shown in previous work, this is the optimal number of persistence fences for lock-free objects~\cite{cohen18}.



% \section{Reaching Optimality}\label{sec:optimality}

% %The attentive reader will notice that our algorithm, presented in Section~\ref{sec:algos}, uses $k+1$ \cas{} instructions to implement a $k$-word \mcas{}; the persistent version of our algorithm additionally uses $2$ persistence fences for the same task. 
% In this section, we describe how our algorithm can be modified to become optimal, both in terms of \cas{} instructions and in terms of persistence fences~\cite{cohen18}.
% Intuitively, the crucial change consists in avoiding the atomic update of the status field of \mcasdescriptor{} (with \cas{}), but rather doing that with a simple store, while ensuring the status of an operation is never ambiguous.

% We introduce a new notion, compared to our algorithm in Section~\ref{sec:algos}, namely, \textit{failure} descriptors.
% Those are structures with the following fields: a pointer $P$ to another descriptor $D$, an address $W$ and a value $V$. 
% As explained below, a failure descriptor is created and used to fail the \mcas{} operation corresponding to $D$.
% We distinguish between a failed and a non-failed (regular) descriptor by stealing one of the least-significant bits in a pointer.
% (Alternatively, we can add an immutable \texttt{type} field in the descriptor structures initialized during the construction of a descriptor).
 
% The new algorithm works as follows.  
% Just like before, an \mcas{} $M$ attempts to lock (install pointers to an \mcasdescriptor{} in) the target words one-by-one, using one \cas{} instruction per locked word.
% $M$ is successful if it manages to lock all its words.
% If $M$ finds a value $V$ different from the expected value $E$ in one of the target words $W$, $M$ creates a failure descriptor (with a pointer $D$, address $W$ and value $V$), and installs (with \cas{}) a pointer to this failure descriptor into $W$. 
% This has the effect of failing $M$.
% Thus, a successful \mcas{} operation would employ exactly $k$ CAS instructions, while a failed \mcas{} would employ at most $k$ CAS instructions. 

% Like before, when a (read or another \mcas{}) operation $M'$ finds a pointer to an active descriptor of \mcas{} $M$,
% it helps $M$ to complete by reading though all $M$'s words (which are sorted by their target addresses, as before), and either 
% installing $M$'s descriptor or $M$'s failure descriptor.
% The traversal immediately stops if $M'$ succeeds to install a failure descriptor, 
% or finds it in one of the $M$'s words.

% After the traversal is done by a thread $T$ (which may be the thread that invoked $M$ or another thread helping $M$), 
% $T$ checks the status of $M$ and sets the status (corresponding to the result of $T$'s traversal) only if the status is not set.
% This check, albeit non-atomic, is crucial for correctness, which follows from the following argument. 
% If a thread manages to lock a word for $M$, then it is either the first to do so, 
% or the lock has been already set up and cleared in the past (by another operation), 
% but then the clearance would happen only after the status is set.
% Note that in the latter case, such a tardy lock is benign, as we can always recover the actual value that the lock replaced from the (failed or regular) descriptor for $M$.

% To complete the description of the modified algorithm, we note that the call for \texttt{retireForCleanup} (see Line~\ref{retire-for-cleanup} in Listing~\ref{list:algo}) 
% is done only by the thread that invoked the corresponding \mcas{} operation.
% This is to prevent multiple threads from reclaiming the same descriptor.
% Finally, we eliminate the persistence fence after updating the status.
% To ensure durable linearizability, however, we need to make sure the status word for $M$ is persisted before unlocking 
% any of $M$'s words.
% We achieve that by flushing $M$'s status and issuing a persistence fence before replacing a pointer to $M$'s descriptor with a pointer to $M'$ descriptor
% (i.e., before executing Line~\ref{mcas-acquire} in Listing~\ref{list:algo}).
% As such, an \mcas{} operation that does not update words currently locked by another \mcas{} operation requires just one persistence fence (see Line~\ref{fence-acquire} in Listing~\ref{list:algo}).
% This fence ensures the persistence of all locked words (in the case of a successful \mcas{}), or the persistence of the failure descriptor (in the case of a failed \mcas{}). 
%  As shown in previous work, this is the optimal number of persistence fences for lock-free objects~\cite{cohen18}.


